Aria Everyday Activities Dataset

We present Aria Everyday Activities (AEA) Dataset, an egocentric multimodal open dataset recorded using Project Aria glasses. AEA contains 143 daily activity sequences recorded by multiple wearers in five geographically diverse indoor locations. Each of the recording contains multimodal sensor data recorded through the Project Aria glasses. In addition, AEA provides machine perception data including high frequency globally aligned 3D trajectories, scene point cloud, per-frame 3D eye gaze vector and time aligned speech transcription. In this paper, we demonstrate a few exemplar research applications enabled by this dataset, including neural scene reconstruction and prompted segmentation. AEA is an open source dataset that can be downloaded from https://www.projectaria.com/datasets/aea/. We are also providing open-source implementations and examples of how to use the dataset in Project Aria Tools https://github.com/facebookresearch/projectaria_tools.

==> figures/aria_data_tools_visualization.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/images/aria_sensors.jpg}
    \caption{The hardware components in the Project Aria form factor. We illustrate the location of each sensor on device, and an example streaming configuration for each sensor. Except the WiFi Bluetooth GNSS were turned off during Aria Everyday Activity recordings, all other sensors are used.}
    \label{fig:aria_device_figure}
\end{figure}

==> figures/speech_prompt.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/images/groundingSAM_example1.png}
    \includegraphics[width=0.45\linewidth]{figures/images/groundingSAM_example2.png}
    \caption{A example showing speech grounded detection using GroundingDino\cite{grounding_dino} and instance segmentation using EfficientSAM\cite{efficientsam}}
    \label{fig:speech_prompt}
\end{figure}

==> figures/time_synchronization.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/images/time_synchronization.png}
    \caption{A snapshot of two synchronized captures at the same timestamp when two wearers playing board games from the opposing views. \todo{substitute it with the rerun visualizer } }
    \label{fig:time_synchronization}
\end{figure}
